Neural Machine Translation for Extremely Low-Resource African Languages: A Case Study on Bambara

Low-resource languages present unique challenges to (neural) machine translation. We discuss the case of Bambara, a Mande language for which training data is scarce and requires significant amounts of pre-processing. More than the linguistic situation of Bambara itself, the socio-cultural context within which Bambara speakers live poses challenges for automated processing of this language. In this paper, we present the first parallel data set for machine translation of Bambara into and from English and French and the first benchmark results on machine translation to and from Bambara. We discuss challenges in working with low-resource languages and propose strategies to cope with data scarcity in low-resource machine translation (MT).

==> donot_touch_this.tex <==
%% fr <---> bam
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lllllll}
        \toprule
        & & & \multicolumn{2}{c}{\textbf{bam$\rightarrow$fr}} & \multicolumn{2}{c}{\textbf{fr$\rightarrow$bam}} \\
         & \textbf{NMT Model} & \textbf{Configuration} & \textbf{BLEU} & \textbf{ChrF} & \textbf{BLEU} & \textbf{ChrF}\\
        \midrule        
         (1) & Word & 2464 (fr) / 1724 (bam) words & 7.7 & 0.2 & 4.9 & 0.1 \\ % Test (not finalized model):   5.91 & 3.37
         (2) & Char & 97 (fr) / 89 (bam) chars & 9.8 & 0.2 & 11.6 & 0.2\\ % Test: 11.55 & 11.15 
         
         \midrule
         (3) & BPE & 500 subword merges each & 18.3 & 0.3 & \textbf{19.8} & 0.3 \\ % Test: 19.36 & 19.70
         (4) & BPE & 1000 subword merges each & \textbf{18.8} & 0.3 & 19.1 & 0.3 \\ % Test: 18.33 &  19.73 
         
         \midrule
         (5) & (3) + BPE dropout & dropout=0.1 & 15.2 & 0.3 & 15.7 &  0.2 \\ % Test: 16.54 & 17.71
         (6) & (4) + BPE dropout & dropout=0.1 & 14.8 & 0.3 & 16.7 & 0.2 \\ % Test: 15.79 & 16.64

         \midrule
       %  (7) & + Backtranslation (BT-F) with fine-tuning &  & & &\\
        % (8) & + Backtranslation (BT-R) with re-training &  & & &\\
        % (9) & + Iterative BT(-F or -R) [whatever works best] & & & &\\
         \midrule
         \multicolumn{2}{l}{\textbf{Test scores} for the best models from above} & & 19.9 & 0.3 & 20.0 & 0.3 \\ % so far: (3), with <pad> replacement
         \bottomrule
    \end{tabular}%
    }
    \caption{NMT results for French and Bambara translations in corpus BLEU and ChrF on the dev set. The best model (in bold) is evaluated on the test set, results are reported in the last row.}
    \label{tab:results_fr}
\end{table*}
% <pad> replacement in model outputs: 
% sed 's/<pad>//g' in > out
% sacrebleu BLEU:
% sacrebleu test.bam --tokenize none < modelhyps.test
% sacrebleu ChrF: 
% sacrebleu test.bam --tokenize none --metrics chrf < modelhyps.test

%% en <---> bam
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lllllll}
        \toprule
        & & & \multicolumn{2}{c}{\textbf{bam$\rightarrow$en}} & \multicolumn{2}{c}{\textbf{en$\rightarrow$bam}} \\
         & \textbf{NMT Model} & \textbf{Configuration} & \textbf{BLEU} & \textbf{ChrF} & \textbf{BLEU} & \textbf{ChrF}\\
        \midrule        
       %  (1) & Word & ?? (en) / ?? (bam) words & -- &  & -- &  \\ % Test (not finalized model):   -- & --
        % (2) & Char & ?? (en) / ?? (bam) chars & -- &  & -- & \\ % Test: -- & -- 
         
    %     \midrule
         (1) & BPE & 500 subword merges each & 17.6 & 0.3 & \textbf{19.13} & 0.3 \\ % Test: 14.12 & 19.14
         (2) & BPE & 1000 subword merges each & \textbf{18.4 }& 0.3 & 17.72 & 0.3 \\ % Test: 13.04 &  18.36 
         
         \midrule
         (3) & (1) + BPE dropout & dropout=0.1 & 14.46 & 0.2 & 15.7 & 0.3 \\ % Test: 11.94 & 17.71
         (4) & (2) + BPE dropout & dropout=0.1 & 12.50 & 0.2 & 16.16 & 0.2 \\ % Test: 11.89 & 16.31

    %     \midrule
    %     (7) & + Backtranslation (BT-F) with fine-tuning &  & & &\\
%         (8) & + Backtranslation (BT-R) with re-training &  & & &\\
%         (9) & + Iterative BT(-F or -R) [whatever works best] & & & &\\
%         \bottomrule
        \midrule
        \midrule
         \multicolumn{2}{l}{\textbf{Test scores} for the best models from above} & &  &  &  &  \\ % so far: (3), with <pad> replacement
         \bottomrule
    \end{tabular}%
    }
    \caption{NMT results for English and Bambara translations in corpus BLEU and ChrF on the dev set. The best model (in bold) is evaluated on the test set, results are reported in the last row.}
    \label{tab:results_en}
\end{table*}

% *****************
% new ****


%% fr <---> bam
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lllllll}
        \toprule
        & & & \multicolumn{2}{c}{\textbf{bam$\rightarrow$fr}} & \multicolumn{2}{c}{\textbf{fr$\rightarrow$bam}} \\
         & \textbf{NMT Model} & \textbf{Configuration} & \textbf{BLEU} & \textbf{ChrF} & \textbf{BLEU} & \textbf{ChrF}\\
        \midrule        
        %  (1) & Word & 2464 (fr) / 1724 (bam) words &  &  &  &  \\ % Test  & 
        %  (2) & Char & 97 (fr) / 89 (bam) chars &  &  &  & \\ % Test:  &  
         (1) & Word & 2464 (fr) / 1724 (bam) words & 7.7 & 0.2 & 4.9 & 0.1 \\ % Test (not finalized model):   5.91 & 3.37
         (2) & Char & 97 (fr) / 89 (bam) chars & 9.8 & 0.2 & 11.6 & 0.2\\ % Test: 11.55 & 11.15 
         
         \midrule
         (1) & BPE & 500 subword merges each & 19.1 & 0.3 & \textbf{21.1} & 0.3 \\ % Test: 22.0  & 21.4
         (2) & BPE & 1000 subword merges each & \textbf{19.2} & 0.3 & 20.4 & 0.3 \\ % Test: 20.9 & 21.2
         
         \midrule
         (3) & (1) + BPE dropout & dropout=0.1 & 17.8 & 0.3 & 16.6 & 0.2  \\ % Test: 17.9 & 18.8
         (4) & (2) + BPE dropout & dropout=0.1 & 16.0 & 0.3 & 17.7 & 0.2 \\ % Test: 18.2 & 18.2

         \midrule
       %  (7) & + Backtranslation (BT-F) with fine-tuning &  & & &\\
        % (8) & + Backtranslation (BT-R) with re-training &  & & &\\
        % (9) & + Iterative BT(-F or -R) [whatever works best] & & & &\\
         \midrule
         \multicolumn{2}{l}{\textbf{Test scores} for the best models from above} & &  &  &  &  \\ % so far: (3), with <pad> replacement
         \bottomrule
    \end{tabular}%
    }
    \caption{NMT results for French and Bambara translations in corpus BLEU and ChrF on the dev set. The best model (in bold) is evaluated on the test set, results are reported in the last row.}
    \label{tab:results_fr}
\end{table*}
% <pad> replacement in model outputs: 
% sed 's/<pad>//g' in > out
% sacrebleu BLEU:
% sacrebleu test.bam --tokenize none < modelhyps.test
% sacrebleu ChrF: 
% sacrebleu test.bam --tokenize none --metrics chrf < modelhyps.test

%% en <---> bam
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lllllll}
        \toprule
        & & & \multicolumn{2}{c}{\textbf{bam$\rightarrow$en}} & \multicolumn{2}{c}{\textbf{en$\rightarrow$bam}} \\
         & \textbf{NMT Model} & \textbf{Configuration} & \textbf{BLEU} & \textbf{ChrF} & \textbf{BLEU} & \textbf{ChrF}\\
        \midrule        
       %  (1) & Word & ?? (en) / ?? (bam) words & -- &  & -- &  \\ % Test (not finalized model):   -- & --
        % (2) & Char & ?? (en) / ?? (bam) chars & -- &  & -- & \\ % Test: -- & -- 
         
    %     \midrule
         (1) & BPE & 500 subword merges each & 18.1 & 0.3 & \textbf{21.3} & 0.3 \\ % Test: 15.9  & 20.9
         (2) & BPE & 1000 subword merges each & \textbf{19.1} & 0.3 & 20.0 & 0.3 \\ % Test: 14.8  &  20.9
         
         \midrule
         (3) & (1) + BPE dropout & dropout=0.1 & 17.0 & 0.2 & 19.3 & 0.3 \\ % Test: 13.5 & 21.6
         (4) & (2) + BPE dropout & dropout=0.1 & 15.2 & 0.2 & 18.2 & 0.2 \\ % Test: 13.7 & 18.2

    %     \midrule
    %     (7) & + Backtranslation (BT-F) with fine-tuning &  & & &\\
%         (8) & + Backtranslation (BT-R) with re-training &  & & &\\
%         (9) & + Iterative BT(-F or -R) [whatever works best] & & & &\\
%         \bottomrule
        \midrule
        \midrule
         \multicolumn{2}{l}{\textbf{Test scores} for the best models from above} & &  &  &  &  \\ % so far: (3), with <pad> replacement
         \bottomrule
    \end{tabular}%
    }
\end{table*}
